Mining Multi-Label Samples from Single Positive Labels

Conditional generative adversarial networks (cGANs) have shown superior results in class-conditional generation tasks. To simultaneously control multiple conditions, cGANs require multi-label training datasets, where multiple labels can be assigned to each data instance. Nevertheless, the tremendous annotation cost limits the accessibility of multi-label datasets in real-world scenarios. Therefore, in this study we explore the practical setting called the single positive setting, where each data instance is annotated by only one positive label with no explicit negative labels. To generate multi-label data in the single positive setting, we propose a novel sampling approach called single-to-multi-label (S2M) sampling, based on the Markov chain Monte Carlo method. As a widely applicable "add-on" method, our proposed S2M sampling method enables existing unconditional and conditional GANs to draw high-quality multi-label data with a minimal annotation cost. Extensive experiments on real image datasets verify the effectiveness and correctness of our method, even when compared to a model trained with fully annotated datasets.

==> 07_Ethics.tex <==
\section{Ethics Statement}

This work demonstrates that it is possible to generate multi-label data from limited labels.
In addition, this work can be freely adopted to unconditional GANs trained with a large amount of unlabeled data.
Hence, our work can reduce the high annotation cost that research groups face in common.
Despite the fact that deep learning models tend to struggle from learning underrepresented data~\citep{abs-1908-09635}, properly calibrated sampling algorithm does not readily ignore rarely appearing data, meaning that it is unlikely to introduce bias into generative models.


==> 08_Reproducibility.tex <==
\section{Reproducibility Statement}

For reproducibility, we provide executable source codes of our proposed S2M sampling with instructions in the Supplementary Material.
